On the Optimal Control of Network LQR with Spatially-Exponential Decaying Structure

This paper studies network LQR problems with system matrices being spatially-exponential decaying (SED) between nodes in the network. The major objective is to study whether the optimal controller also enjoys a SED structure, which is an appealing property for ensuring the optimality of decentralized control over the network. We start with studying the open-loop asymptotically stable system and show that the optimal LQR state feedback gain $K$ is `quasi'-SED in this setting, i.e. $\|[K]_{ij}\|\sim O\left(e^{-\frac{c}{\mathrm{poly}\ln(N)}}\mathrm{dist}(i,j)\right)$. The decaying rate $c$ depends on the decaying rate and norms of system matrices and the open-loop exponential stability constants. Then the result is further generalized to unstable systems under a SED stabilizability assumption. Building upon the `quasi'-SED result on $K$, we give an upper-bound on the performance of $\kappa$-truncated local controllers, suggesting that distributed controllers can achieve near-optimal performance for SED systems. We develop these results via studying the structure of another type of controller, disturbance response control, which has been studied and used in recent online control literature; thus as a side result, we also prove the `quasi'-SED property of the optimal disturbance response control, which serves as a contribution on its own merit.

==> Sections/Relationship-to-state-feedback.tex <==
\section{Relationship to optimal state feedback control gain}\label{sec:translate-back-to-state-feedback}
The previous section proves that the optimal disturbance feedback $\LK$ has the SED structure. As an immediate next step, we seek to translate the SED structure on $\LK$ to the optimal state feedback gain $K$. This requires us to look into the the algebraic relation between $\LK$ and $K$. Surprisingly, we found that $-\LK_1$ is a good approximation of $K$, which is stated in the following lemma.
\begin{lemma}\label{lemma:relationship-K-L} 
Let $K$ be the optimal control gain of the corresponding LQR problem, then $\LK$ solved from \eqref{eq:L-tilde-eq} satisfies
\begin{equation}
    \|K + L_1^{(H)}\| \le \frac{2\tau^3(\|B\|^2\|K\|\|Q\|+\|B\|\|K\|\|S\|)}{\lmin(R\!-\!SQ^{-1}S^\top)(1-e^{-2\rho})^{5/2}}e^{-H\rho}.
\end{equation}
\end{lemma}
Due to space limit, we defer the intuition and proof of Lemma \ref{lemma:relationship-K-L} to Appendix \ref{apdx:relationship-K-L}. Given this lemma, the SED structure of $\LK$ in Theorem \ref{theorem:spatially-decay-L} can be easily translated to the optimal control gain $K$, and thus obtain Theorem \ref{theorem:spatial-decay-F} (detailed derivation see Appendix \ref{apdx:proof-SED-F}).

% \begin{theorem}[Main result 2, SED structure of $K$]\label{theorem:spatial-decay-F}
% Under Assumption \ref{assump:exponential-decay} and \ref{assump:A-exponential-stable}, the optimal control gain $K$ for problem \eqref{eq:LQR} is $(c_K,\gamma_K)$-SED, where 
% \begin{align*}
%     c_K &\lesssim O\bigg(\textup{poly}\Big(N, \tau,\frac{1}{1-e^{-2\rho}}, \frac{1}{\lmin(R\!-\!SQ^{-1}S^\top)},\\
%     &\qquad \qquad\qquad\qquad\|B\|,\|Q\|,\|S\|,\|K\|, b, q, s\Big)\bigg), \\
%     \gamma_K &\gtrsim  \gammasys \rho\bigg\slash O\bigg(\textup{poly}\Big(\tau,\frac{1}{1-e^{-2\rho}},\frac{1}{\lmin(R\!-\!SQ^{-1}S^\top)},\\
%     &\qquad\quad\!\!\lmax(R),\|B\|,\|Q\|,\|S\|,\ln\left\{N,a,b,q,r,s,\gammasys \right\}\Big)\bigg)\!.
% \end{align*}
% \end{theorem}
% \noindent\textbf{Extension to the unstable $A$ case:} Theorem \ref{theorem:spatial-decay-F} can be extended to the case where $A$ is unstable, or stable but with too small an exponential factor $\rho$ (that possibly scale with, e.g. $1/N$, which makes the bound invalid), under an additional mild assumption on the stabilizability:
% \begin{assump}[Stabilizability of the system]\label{assump:stabilizability}
% There exists a $K_0 \in \mathbb{R}^{n_u\times n_x}$ that is $(k_0, \gammasys )$-SED such that $A-BK_0$ is $(\tau, e^{-\rho})$-stable.
% \end{assump}
% \begin{coro}[of Theorem~\ref{theorem:spatial-decay-F}, extension to unstable case]\label{coro:spatial-decay-F-unstable-A}
% Under Assumption \ref{assump:exponential-decay} and \ref{assump:stabilizability}, and that the system is closed-loop stable, i.e. $A-BK$ is $(\tau,e^{-\rho})$-stable, the optimal control gain $K$ of problem \eqref{eq:LQR} is $(c_K,\gamma_K)$-SED, where 
% \begin{align*}
%     c_K &\lesssim O\bigg(\textup{poly}\Big(N, \tau,\frac{1}{1-e^{-2\rho}}, \frac{1}{\lmin(R\!-\!SQ^{-1}S^\top)},\frac{1}{\lmin(Q)}\\
%     &\qquad \qquad\quad\|B\|,\|Q\|,\|R\|,\|S\|,\|K\|,\|K_0\|^2, b, q, r, s, k_0\Big)\bigg), \\
%     \gamma_K &\gtrsim  \gammasys \rho\!\bigg\slash\! O\!\bigg(\!\textup{poly}\Big(\tau,\frac{1}{1\!-\!e^{\!-\!2\rho}},\frac{1}{\lmin\!(R\!-\!SQ^{-1}S^\top)},\frac{1}{\lmin\!(Q)}\\
%     &\hspace{-4pt}\lmax\!(R),\|B\|,\|Q\|,\|R\|,\|S\|,\|K_{\!0}\|^2,\ln\!\left\{\!N\!,a\!,b\!,q\!,r\!,s\!,k_0\!,\gammasys \!\right\}\!\!\Big)\!\!\bigg)\!.
% \end{align*}
% \end{coro}
% The proofs of Theorem \ref{theorem:spatial-decay-F} and Corollary \ref{coro:spatial-decay-F-unstable-A} are deferred to Appendix \ref{apdx:proof-SED-F}. 

% We would refer the reader to the previous section for the discussion of the decay rate $\gamma_K^{(K)}$ , which is very similar to $\gamma_L^{(K)}$ (Remark \ref{rmk:SED-rate-validness} and \ref{rmk:decay-rate}). Here we provide one toy example to justify the usefulness of the result.

% %{\color{blue} Change this accordingly}
% \begin{example}[Heat equation revisited]\label{example:toy}
% Similar to Example \ref{example:circle}, we consider the same circle graph $\mathbb{Z}_N$ and consider heat equation. For the sake of simplicity, here we consider a simpler form of discretization than \eqref{eq:discretization} (however, similar results can be obtained for discretization \eqref{eq:discretization}), i.e.,
% \begin{equation*}
%      x_{t+1}^i =  x_t^i + \eta\left(-2x_t^i + x_t^{i+1} + x_t^{i-1}  + u_t^i\right),
% \end{equation*}
% where $\eta >0$ are some constant. Thus $A = I-\eta L$, where $L$ is graph Laplacian of  $\mathbb{Z}_N$, and $B = I$. From now on we assume that $\eta$ is small enough such that $A$ is a positive-semi-definite matrix, i.e., $\eta \le \frac{1}{4}$.
% The control objective is to let the state vector goes to zero while keeping the control energy low, which we set as
% \begin{equation*}
%     \min \lim_{T\to\infty}\frac{1}{T} \sum_{t=1}^T\sum_{i=1}^N  {x_t^i}^2 + \alpha {u_t^i}^2,
% \end{equation*}
% thus $Q, R$ matrices in this setting are $Q = I, R = \alpha I, S=0$.

% Note that $A$ is not exponentially stable as it has $1$ as its eigenvalue (the all-one vector is its corresponding eigenvector). Thus Theorem \ref{theorem:spatial-decay-F} is not directly applicable. Yet we could set $K_0 = \frac{1}{2}I$, and $A-BK_0 = \frac{1}{2} I-\eta L \Longrightarrow \|A-BK_0\|\le \frac{1}{2}$, i.e., $A-BK_0$ is $(1,\ln(2))$-stable, hence Assumption \ref{assump:stabilizability} is satisfied and Corollary \ref{coro:spatial-decay-F-unstable-A} can be applied.

% In this example, we can set $\gammasys  = \log(\frac{1}{\eta}), a=1, b=1, q=1, r=\max\{\alpha,1\}$ in Assumption \ref{assump:exponential-decay}, and set $\tau = 1$, $\rho = \ln 2$,$\|K_0\| = 1/2$, $f = 1/2$ in Assumption \ref{assump:stabilizability}. Additionally, the system norms are bounded by $\|B\|=1, \|Q\|=1, \lmax(R) = \lmin(R)=\alpha$. Note that all these terms are constants that does not depend on the number of agents $N$, thus for any $\mathbb{Z}_N$, $\gamma_K$ in Theorem \ref{theorem:spatial-decay-F} is on the scale $\gamma_K \gtrsim \frac{c}{\ln(N)}$, where $c$ is some constant that does not depend on $N$, which implies that the optimal $K$ for this example is indeed quasi-SED.

% \end{example}

% \subsection{Performance of the truncated controller}
% %\textcolor{blue}{Bookmark: I am here (Results need to be modified both for the main text and the appendix because now we have a bilinear term)}

% This section looks into the performance of the following truncated controller:
% \begin{equation*}
%     [\Ftrunc]_{ij} = \left\{
%     \begin{array}{ll}
%         [K]_{ij} & \textup{if } \dist(i,j)\le \kappa-1 \\
%          0& \textup{otherwise} 
%     \end{array}
%     \right..
% \end{equation*}

% We measure the performance in terms of the LQR cost, i.e., for any exponentially stable controller $K'$, we can define its cost $C(K')$ as:
% \begin{equation*}
% \begin{split}
% C(K') :=\min_{\{u_t\}_{t=0}^{\infty}}&\lim_{T\to\infty} \frac{1}{T}\mathbb{E}\sum_{t=0}^{T-1}x_t^\top Q x_t + u_t^\top Ru_t + 2u_t^\top Sx_t\\
%  s.t.~~ x_{t+1} &= Ax_t + Bu_t + w_t, ~~w_t\sim\mathcal{N}(0,I),\\
% u_t &= K'x_t
% \end{split}
% \end{equation*}

% \begin{theorem}\label{theorem:performance-truncated}
% Assume that the optimal control gain $K$ is $(c_K, \gamma_K)$-SED, then for $\kappa \ge \frac{\ln\left(\frac{2\tau c_K\sqrt{N}\|B\|}{1-e^{-\rho}}\right)}{\gamma_K},$
% % \begin{equation*}
% %     \kappa \ge \frac{\ln\left(\frac{2\tau c_K\sqrt{N}\|B\|}{1-e^{-\rho}}\right)}{\gamma_K},
% % \end{equation*}
% we have that
% \begin{equation*}
% \begin{split}
% &\quad C(\Ftrunc) - C(K) \\
% &\le \frac{2\tau}{1-e^{-\rho}} \|R+B^\top P B\|\sqrt{N\min\{n_x,n_u\}} c_K e^{-\gamma_K\kappa},
% \end{split}
% \end{equation*}
% where $P$ is defined in \eqref{eq:ricatti-eq}.
% \end{theorem}

